Counterexample Classification

In model checking, when a given model fails to satisfy the desired specification, a typical model checker provides a counterexample that illustrates how the violation occurs. In general, there exist many diverse counterexamples that exhibit distinct violating behaviors, which the user may wish to examine before deciding how to repair the model. Unfortunately, obtaining this information is challenging in existing model checkers since (1) the number of counterexamples may be too large to enumerate one by one, and (2) many of these counterexamples are redundant, in that they describe the same type of violating behavior. In this paper, we propose a technique called counterexample classification. The goal of classification is to partition the space of all counterexamples into a finite set of counterexample classes, each of which describes a distinct type of violating behavior for the given specification. These classes are then presented as a summary of possible violating behaviors in the system, freeing the user from manually having to inspect or analyze numerous counterexamples to extract the same information. We have implemented a prototype of our technique on top of an existing formal modeling and verification tool, the Alloy Analyzer, and evaluated the effectiveness of the technique on case studies involving the well-known Needham-Schroeder protocol with promising results.

==> sections/Section8-Acknowledgements.tex <==
This work has been supported by the National Science Foundation under NSF SaTC award CNS-1801546.


==> sections/figures/classify.tex <==
\begin{figure}[t]
  \begin{algorithm}[H]
    \SetKwProg{Fn}{Func}{}{}
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{an $\sts$, a specification $\Phi$, and a set of predicates $V$}
    \Output{a set of trace constraints $W$}
    \Fn{$\classify(\sts, \Phi, V)$:}{
      $W = \emptyset$\;
      \While{$\verify(\sts, W, \Phi)$ == $\nok$}{
        $\rho$ = $\counterexample(\sts, W, \Phi)$\;
        $\Gamma$ = $\facts(\rho, V)$\;
        \If{$\Gamma = \emptyset$}{
          \KwRet{``The given $V$ cannot generate any facts for $\rho$''}
        }
        $w$ = $\traceConstraint(\Gamma, \rho)$\;
        \If{$c(w) \cap \Phi \ne \emptyset$}{
          \KwRet{``The given $V$ cannot characterize the behavior of $\rho$''}
        }
        $W$ = $W \cup w$\;
      }
      \KwRet{$W$}\;
    }
    \caption{The basic counterexample classification algorithm.}
    \label{alg-classify}
  \end{algorithm}
\end{figure}


==> sections/figures/classifyOpt.tex <==
\begin{figure}
  \begin{algorithm}[H]
    \SetKwProg{Fn}{Func}{}{}
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{an $\sts$, a specification $\Phi$, and a set of predicates $V$}
    \Output{a set of trace constraints $W$}
    \Fn{$\classifyOpt(\sts, \Phi, V$):}{
      $W = \emptyset$\;
      \While{$\verify(\sts, W, \Phi)$ == SAT}{
        $\rho$ = $\counterexample(\sts, W, \Phi)$\;
        $\Gamma$ = $\facts(\rho, V)$\;
        \If{$\Gamma = \emptyset$}{
          \KwRet{``The given $V$ cannot classify all violating behaviors''}
          }
        $w$ = $\traceConstraint(\Gamma, \rho)$\;
        \If{$c(w) \cap \Phi \ne \emptyset$}{
          \KwRet{``The given $V$ cannot characterize the violating behavior of $\rho$''}
        }
        $w$ = $\minimizetc(\sts, w, \Phi)$\;
        $W$ = $W \cup w$\;
      }
      $W$ = $\redundancyCheck(W)$\;
      \KwRet{$W$}\;
    }
    \caption{Optimized counterexample classification algorithm.}
    \label{alg-classifyOpt}
  \end{algorithm}
\end{figure}


==> sections/figures/counterexamples.tex <==
\begin{adjustbox}{max totalsize={1.0\textwidth}{.3\textheight}}

  \newcommand\height{0.5cm}
  \newcommand\width{4cm}
  \begin{tikzpicture}[->, >=stealth', shorten >=1pt, auto, semithick]

  \tikzstyle{every state} = [minimum size=1.8cm, inner sep=0pt, align=center]
  \tikzstyle{every node} = [font=\small]
  
  \node[state, label={[xshift=-4em, yshift=-3.3em]\normalsize $\rho_1$}]  (q0_0) 
    {$\{ \emptyset, F\}$};
  \node[state] (q0_1)
    [right=\width of q0_0] 
    {$\{\emptyset, T\}$};
  
  \path (q0_0) 
    edge [right] node[pos=0.5, above]
            {$(\Plaintext, Alice, T)$}
            (q0_1);

  %%%%%%%%%%%%%%%%%%%%%

  \node[state, label={[xshift=-4em, yshift=-3.3em]\normalsize $\rho_2$}]  (q0_1) 
    [below=\height of q0_0] 
    {$\{\emptyset, F\}$};
  \node[state] (q1_1)
    [right=\width of q0_1] 
    {$\{\emptyset, T\}$};

  \path (q0_1) 
    edge [right] node[pos=0.5, above]
            {$(\Plaintext, Bob, T)$}
            (q1_1);

  %%%%%%%%%%%%%%%%%%%%%

  \node[state, label={[xshift=-4em, yshift=-3.3em]\normalsize $\rho_3$}]  (q0_2) 
    [below=\height of q0_1] 
    {$\{\emptyset, F\}$};
  \node[state] (q1_2)
    [right=\width of q0_2] 
    {$\{Key_{AB}, F\}$};
  \node[state] (q2_2)
    [right=\width of q1_2] 
    {$\{Key_{AB}, T\}$};

  \path (q0_2) 
          edge [right] node[pos=0.5, above]
            {$(\Encrypted, Alice, F)$}
            (q1_2)
        (q1_2)
          edge [right] node[pos=0.5, above]
            {$(\Encrypted, Bob, T)$}
            (q2_2);
    
  
  %%%%%%%%%%%%%%%%%%%%%

  \node[state, label={[xshift=-4em, yshift=-3.3em]\normalsize $\rho_4$}]  (q0_3) 
    [below=\height of q0_2]
    {$\{ \emptyset, F\}$};
  \node[state] (q1_3)
    [right=\width of q0_3] 
    {$\{Key_{AB}, F\}$};
  \node[state] (q2_3)
    [right=\width of q1_3] 
    {$\{Key_{AB}, T\}$};

  \path (q0_3) 
          edge [right] node[pos=0.5, above]
          {$(\Encrypted, Alice,T)$}
          (q1_3)
        (q1_3)
          edge [right] node[pos=0.5, above]
          {$(\Encrypted, Alice,T)$}
          (q2_3);
  
  %%%%%%%%%%%%%%%%%%%%%
  
  \node[state, label={[xshift=-4em, yshift=-3.3em]\normalsize $\rho_5$}]  (q0_4) 
    [below=\height of q0_3]
    {$\{ \emptyset, F\}$};
  \node[state] (q1_4)
    [right=\width of q0_4] 
    {$\{Key_{AB}, F\}$};
  \node[state] (q2_4)
    [right=\width of q1_4] 
    {$\{Key_{AB}, T\}$};

  \path (q0_4) 
          edge [right] node[pos=0.5, above]
          {$(\Encrypted, Alice,T)$}
          (q1_4)
        (q1_4)
          edge [right] node[pos=0.5, above]
          {$(\Plaintext, Alice,T)$}
          (q2_4);

\end{tikzpicture}
\end{adjustbox}

==> sections/figures/facts.tex <==

\begin{figure}
    \begin{algorithm}[H]
      \SetKwInOut{Input}{Input}
      \SetKwInOut{Output}{Output}
      \Input{a counterexample $\rho$ and a set of predicates $V$}
      \Output{set of true instantiations of each $v \in V$ at each state in $\rho$}
      \SetKwProg{Fn}{Func}{}{}
      \DontPrintSemicolon
      \Fn{$\facts(\rho, V$):}{
        $\Gamma$ = $\emptyset$\;
        \For{$v, s \in V, \states(\rho) \mbox{ such that } typecheck(v, s)$}{
          \For{$i \in [0..len(\rho)]$}{
            \If{$eval(v(s@i))$}{
              $\Gamma$ = $\Gamma \cup v(s@i)$\;
            }
          }
        }
        \KwRet{$\Gamma$}\;
      }
      \caption{The $\facts$ procedure.}
	  \label{algo_facts}
    \end{algorithm}
  \end{figure}

==> sections/figures/runningTimeTable.tex <==
\begin{table}
  \title{Spent Time}
  \centering
  \begin{tabular}{|c|c|c|c|}
    \hline
    Command Run & Running Time (min) \\\hline
    Check and Found NO Counterexample   &   2.66   \\\hline  
    Check and Found Counterexample &   2.64   \\\hline  
    Check and Found Counterexample &   2.61   \\\hline    
    Check and Found NO Counterexample   &   2.4    \\\hline  
    Check and Found Counterexample &   2.2    \\\hline  
    Check and Found NO Counterexample   &   2.1    \\\hline  
    Check and Found NO Counterexample   &   2.0    \\\hline  
    Check and Found Counterexample &   1.9    \\\hline 
    Check and Found Counterexample &   1.76   \\\hline 
    Successful Subsumption Check         &   1.03 \\\hline
  \end{tabular}
  \caption{Typical run of the Symmetric model listing the ten most
    time-intensive commands.\eunsuk{This table probably needs some
      more explanation. What do these different rows represent, and
      why do some of them have the same name?}}
  \label{table:timeSpent}
\end{table}

